Transfer Reinforcement Learning in Heterogeneous Action Spaces using Subgoal Mapping

In this paper, we consider a transfer reinforcement learning problem involving agents with different action spaces. Specifically, for any new unseen task, the goal is to use a successful demonstration of this task by an expert agent in its action space to enable a learner agent learn an optimal policy in its own different action space with fewer samples than those required if the learner was learning on its own. Existing transfer learning methods across different action spaces either require handcrafted mappings between those action spaces provided by human experts, which can induce bias in the learning procedure, or require the expert agent to share its policy parameters with the learner agent, which does not generalize well to unseen tasks. In this work, we propose a method that learns a subgoal mapping between the expert agent policy and the learner agent policy. Since the expert agent and the learner agent have different action spaces, their optimal policies can have different subgoal trajectories. We learn this subgoal mapping by training a Long Short Term Memory (LSTM) network for a distribution of tasks and then use this mapping to predict the learner subgoal sequence for unseen tasks, thereby improving the speed of learning by biasing the agent's policy towards the predicted learner subgoal sequence. Through numerical experiments, we demonstrate that the proposed learning scheme can effectively find the subgoal mapping underlying the given distribution of tasks. Moreover, letting the learner agent imitate the expert agent's policy with the learnt subgoal mapping can significantly improve the sample efficiency and training time of the learner agent in unseen new tasks.

==> tex/Introduction.tex <==
Transfer learning in reinforcement learning has become a topic of vast interest in recent years. With the continual growth of deep learning to improve computation, previous papers in literature have been able to show many algorithms that can improve the speed of learning for an agent once it learns from an already trained agent. Transfer learning has been used in a variety of applications, spanning from speech recognition [14], imaging [5], and even gaming [9]. Although the transfer learning space is vast, the idea of "knowledge distillation" [] is prevalent across these methods, where " " []. With deep learning, transfer methods can extract important abstract information in the hopes of passing it on to another, often simpler, agent.

A common feature in most transfer learning methods is the use of KL divergence to help train the second agent who seeks to learn from the first agent who has already learned an optimal policy. KL divergence measures the difference between two distributions and therefore is a natural quantity to minimize when trying to ensure information has been passed on. However, this general approach has limitations when trying to transfer across agents who might have different action spaces. 

The ability to transfer knowledge across different action spaces would be incredibly helpful when training heterogeneous groups of agents. Instead of having to train each type of agent, an expert agent's policy could be transferred to any other type of agent, thereby decreasing overall training time. In fact, this ability can also be quite useful among homogeneous groups as well. If a certain agent is damaged and its action space becomes more limited or changes in any way, transferring existing knowledge from other agents in the group can still add value to the damaged agent, which could mean increasing its time in the field before it needs to be repaired, increasing overall output of the group of agents.

Such use cases motivate the use of few-shot learning for this problem, where an agent attempts to learn a policy having received only a few expert demonstrations \cite{oneshot}. A few-shot approach can help as information overload in the event of too many expert demonstrations might not be as helpful, especially as any information that is being transferred across different action spaces will be abstract.

Existing methods who seek to solve this problem have tried a variety of solutions. [6] uses a modular approach where they decompose neural network policies into "task-specific" and "robot-specific" modules, the former being shared across robots and the latter shared across all tasks on that agent. However, this method requires explicit meshing of modules together to find an optimal policy, and in very complex environments this is not a trivial task.

[16] uses a handcoded mapping between different tasks which has parallels to the case of different action spaces, as in both cases having a mapping would be quite useful in terms of transferring information. [] also uses a handcoded mapping, but were not able to get competitive experimental results. Although handcoded mappings have been proven to work in some capacity, we can see that human crafted ones have the weakness of being suboptimal as well as not being automatically generated leading to more setup work before one begins the process of transfer learning.

\cite{imithetero} seeks to learn a policy from an expert even under sparse reward conditions, choosing when to imitate the expert and when to explore by itself. However, their method is highly dependent on self-exploration of the learner as many of their results seem to be dominated by the learner agent self-exploring and finding better trajectories rather than choosing to listen to the expert. 

[19] to our knowledge is the most state-of-the-art in terms of transfer learning between different action spaces, even being able to transfer between state spaces. However, we see their approach as more architectural, as they seek to blend aspects of the teacher network into the student network by sharing policy parameters, whereas we believe an approach that is less dependent on explicitly blending together networks can be adapted easier in most environments.
%Multi-Agent Reinforcement Learning (MARL) has been recently used to solve large-scale decision making problems in a variety of application domains, including cyber-physical systems \cite{multiagentrloverview}, financial systems \cite{stocktradingcooprl}, and strategic games \cite{ddpgtransferstarcraftmicro, multiobjcoopcoevrtsmicro}. The goal is to enable a team of agents to collaboratively determine a global optimal policy that maximizes the sum of their local accumulated rewards. Nevertheless, perhaps the main limitation of existing MARL methods is that they are still computationally very expensive and require many iterations to converge \cite{maactorcriticmixedcoopcompenv}. In this paper, we propose a new distributed off-policy actor-critic method for MARL that relies on augmented Lagrangian (AL) optimization to significantly improve the convergence rate compared to existing methods in the literature.

%A major challenge in MARL is to coordinate agents with consensus constraints. This category of problems require agents' policies to be consistent with their respective positions and relationships within the graph network, and can be applicable in environments that require time-sensitive information transfer or for synchronized teamwork. Centralized methods that seek to coordinate agents from a master node have not been popular due to an inability to scale (curse of dimensionality [5]) and a large dependence on communication due to many agents seeking to communicate with the central coordinator. As a result, decentralized methods are preferred [6, 7]. Within a decentralized approach, methods can either be value based [8] or use policy gradients [9]. 

%Distributed MARL \color{blue}policy evaluation methods can make learning unstable and break any convergence guarantees \cite{meanfieldmarl}. \color{black} As a result, policy gradient methods have been preferred \cite{multisoftqlearn}. Policy gradient methods do not typically encounter the same stability issues as these methods focus on optimizing any parameters of interest directly and are also stable under function approximation given a sufficiently small learning rate \cite{bridgegapvaluepolrl}.

%A popular class of MARL policy gradient methods is the multi-agent Actor-Critic method \cite{diffdac,yanpaper} in which each agent has a Critic component which evaluates the current policy and an Actor component which updates the agent's policy using a gradient ascent step. In \color{red}[...] \color{black}, an Actor Critic method is extended to a MARL setting by letting all the agents estimate the global Critic function in a fully distributed way. Specifically, \color{red} [17] \color{black} applies the gossip algorithm and \color{red} [18, 20] \color{black} applies averaging schemes so that all the agents reach consensus on their Critic functions. However, these works require the agents to share local rewards or value functions with their neighbors at each time instant in each episode, which may raise privacy concerns and induce large communication overhead.\color{black}

%Existing Actor-Critic methods for MARL parameterize the state-action value function, and they typically rely on temporal difference methods to update the Critic and consensus methods to share the information needed to update the Actor [11, 16]. Specifically, gossip algorithms [17] and other averaging schemes [18-20] have been proposed to update the Actor but these methods require each agent share its local task information such as local rewards or value functions, multiple times throughout an entire episode.

%To reduce the number of iterations and communication rounds in distributed Actor-Critic methods, a different class of methods have been proposed that use optimization techniques to update the Actor. As mentioned earlier, we propose a distributed Augmented Lagrangian method in order to update our Actor step.
%Rather than keeping consensus on global Critic estimates, \color{red} [6, 21, 22] \color{black} let all agents update their Actor functions with the policy gradients of their local value functions, share their Actor parameters with their neighbors and achieve consensus on the local Actor functions. Such a consensus Actor scheme only requires communication at the end of each episode and do not need the agents to share their task information, e.g., local rewards and value functions. However, these methods fall into the class of consensus gradient methods \color{red}[ref] \color{black} and result in a slow convergence rate when the value function of the problem is nonsmooth. To accelerate the convergence and improve the sampling efficiency, in this paper, we employ the distributed augmented Lagrangian (AL) technique on the local Actor updates and develop a novel distributed Actor Critic method. Rather than solving an inner optimization problem at each time step in existing distributed AL methods \color{red}[ref]\color{black}, we approximate the solution of the inner problem by updating the local Actor with one gradient step. Such updates require unbiased local policy gradient estimates, which are obtained by adopting the emphatic policy gradient under the MARL setting. Convergence of the proposed method is established theoretically.

%Compared to consensus-based Critic methods that require sharing value function parameters multiple times during every episode, our proposed method only requires the policy parameters to be shared at the end of each episode which can reduce sample complexity.
%Perhaps the most related works are \color{red}[23, 5]\color{black}. In \color{red}[23]\color{black}, the authors formulate the consensus constraints on the local Actor parameters and apply the dual decomposition method to update local Actor parameters. However, dual decomposition method usually suffers from slow convergence rate. The works in \color{red}[5]\color{black} apply the ADMM algorithm to deal with the Actor consensus constraints. However, no convergence analysis is provided and the algorithm implementation requires a fully connected communication graph. \color{black}

%Perhaps most closely related to the method proposed is the approach in [23] which implements a distributed policy gradient method using dual decomposition while [5] proposes using an ADMM framework. However, in practice, AL optimization converges faster than dual decomposition [24]. Moreover, the ADMM-based approach in [5] is not supported by theoretical convergence results and it also requires the communication graph to be fully connected. Compared to these works, our distributed policy optimization method, is more sample-and communication-efficient. Moreover, we provide theoretical convergence results of our distributed policy gradient algorithm that rely on a two time-scale analysis. This makes our analysis unique when compared to existing AL methods for standard optimization problems [25 - 27].

The rest of the paper is organized as follows. In Section II, we formulate the transfer learning across different action spaces problem under consideration and introduce some preliminaries. In Section III, we propose our algorithm. In Section IV, we show our experimental results along with comparisons with established methods in literature. In Section V, we conclude the paper and discuss future steps.
